Finding the Perfect Fit: Applying Regression Models to ClimateBench v1.0

Climate projections using data driven machine learning models acting as emulators, is one of the prevailing areas of research to enable policy makers make informed decisions. Use of machine learning emulators as surrogates for computationally heavy GCM simulators reduces time and carbon footprints. In this direction, ClimateBench [1] is a recently curated benchmarking dataset for evaluating the performance of machine learning emulators designed for climate data. Recent studies have reported that despite being considered fundamental, regression models offer several advantages pertaining to climate emulations. In particular, by leveraging the kernel trick, regression models can capture complex relationships and improve their predictive capabilities. This study focuses on evaluating non-linear regression models using the aforementioned dataset. Specifically, we compare the emulation capabilities of three non-linear regression models. Among them, Gaussian Process Regressor demonstrates the best-in-class performance against standard evaluation metrics used for climate field emulation studies. However, Gaussian Process Regression suffers from being computational resource hungry in terms of space and time complexity. Alternatively, Support Vector and Kernel Ridge models also deliver competitive results and but there are certain trade-offs to be addressed. Additionally, we are actively investigating the performance of composite kernels and techniques such as variational inference to further enhance the performance of the regression models and effectively model complex non-linear patterns, including phenomena like precipitation.

==> bib.tex <==
\begin{thebibliography}{00}
\bibitem{b1}Ajagekar, A., \& You, F. (2022). Quantum computing and quantum artificial intelligence for renewable and sustainable energy: A emerging prospect towards climate neutrality. Renewable and Sustainable Energy Reviews, 165, 112493. https://doi.org/10.1016/J.RSER.2022.112493
\bibitem{b2} Ayala, A., Drazic, C., Hutchinson, B., Kravitz, B., \& Tebaldi, C. (2021). Loosely Conditioned Emulation of Global Climate Models With Generative Adversarial Networks. http://arxiv.org/abs/2105.06386
\bibitem{b3} Bagnell, D., Narayanan, V., Koval, M., \& Parashar, P. (n.d.). Gaussian Processes (Vol. 12). http://www.gaussianprocess.org/gpml/
\bibitem{b4} Bastos, L. S., \& O’hagan, A. (2009a). Diagnostics for gaussian process emulators. Technometrics, 51(4), 425–438. https://doi.org/10.1198/TECH.2009.08019
\bibitem{b5} Beusch, L., Gudmundsson, L., \& Seneviratne, S. I. (2020). Emulating Earth system model temperatures with MESMER: From global mean temperature trajectories to grid-point-level realizations on land. Earth System Dynamics, 11(1), 139–159. https://doi.org/10.5194/esd-11-139-2020
\bibitem{b6} Beusch, L., Nicholls, Z., Gudmundsson, L., Hauser, M., Meinshausen, M., \& Seneviratne, S. I. (2022). From emission scenarios to spatially resolved projections with a chain of computationally efficient emulators: coupling of MAGICC (v7.5.1) and MESMER (v0.8.3). Geoscientific Model Development, 15(5), 2085–2103. https://doi.org/10.5194/gmd-15-2085-2022
\bibitem{b7} Böhning-Gaese, K., \& Lemoine, N. (2004). Importance of Climate Change for the Ranges, Communities and Conservation of Birds. Advances in Ecological Research, 35, 211–236. https://doi.org/10.1016/S0065-2504(04)35010-5
\bibitem{b8} Camps-Valls, G., Reichstein, M., Zhu, X., \& Tuia, D. (2020). ADVANCING DEEP LEARNING FOR EARTH SCIENCES: FROM HYBRID MODELING TO INTERPRETABILITY. IGARSS 2020 - 2020 IEEE International Geoscience and Remote Sensing Symposium, 3979–3982. https://doi.org/10.1109/IGARSS39084.2020.9323558
\bibitem{b9} Chen, M., Lin, S., Guo, G.-D., \& Li, J. (2021). Quantum Gaussian process regression.
\bibitem{b10} Coleman-Smith, C. E., Müller, B., Robert, S., Steen, W., Bass, A., Chandrasekharan, S., \& Kruse, M. (n.d.). Using Gaussian Processes for the Calibration and Exploration of Complex Computer Models.
\bibitem{b11} De, A. G., Matthews, G., Nickson, T., Fujii, K., Boukouvalas, A., León-Villagrá, P., Ghahramani, Z., \& Hensman, J. (2017). GPflow: A Gaussian Process Library using TensorFlow Mark van der Wilk. In Journal of Machine Learning Research (Vol. 18). http://jmlr.org/papers/v18/16-537.html.
\bibitem{b12} Duvenaud, D. (n.d.). The Kernel Cookbook: Advice on Covariance functions. https://www.cs.toronto.edu/~duvenaud/cookbook/
\bibitem{b13} González-Abad, J., Bã No-Medina, J., \& Manuel Gutiérrez, J. (n.d.). TESTING INTERPRETABILITY TECHNIQUES FOR DEEP STATISTICAL CLIMATE DOWNSCALING. https://www.ecmwf.int/
\bibitem{b14} Hensman, J., Fusi, N. O., \& Lawrence, N. D. (n.d.). Gaussian Processes for Big Data.
\bibitem{b15} Holden, P. B., Edwards, N. R., Garthwaite, P. H., Fraedrich, K., Lunkeit, F., Kirk, E., Labriet, M., Kanudia, A., \& Babonneau, F. (2014). PLASIM-ENTSem v1.0: A spatiooral emulator of future climate change for impacts assessment. Geoscientific Model Development, 7(1), 433–451. https://doi.org/10.5194/gmd-7-433-2014
\bibitem{b16} Karpatne, A., Atluri, G., Faghmous, J. H., Steinbach, M., Banerjee, A., Ganguly, A., Shekhar, S., Samatova, N., \& Kumar, V. (2017). Theory-guided data science: A new paradigm for scientific discovery from data. IEEE Transactions on Knowledge and Data Engineering, 29(10), 2318–2331. https://doi.org/10.1109/TKDE.2017.2720168
\bibitem{b17} Kumar, N., Tischbein, B., Kusche, J., Laux, P., Beg, M. K., \& Bogardi, J. J. (2017). Impact of climate change on water resources of upper Kharun catchment in Chhattisgarh, India. Journal of Hydrology: Regional Studies, 13, 189–207. https://doi.org/10.1016/j.ejrh.2017.07.008
\bibitem{b18} Lalchand, V., Tazi, K., Cheema, T. M., Turner, R. E., \& Hosking, S. (2022). Kernel Learning for Explainable Climate Science. http://arxiv.org/abs/2209.04947
\bibitem{b19} Liu, H., Ong, Y. S., Shen, X., \& Cai, J. (2020). When Gaussian Process Meets Big Data: A Review of Scalable GPs. IEEE Transactions on Neural Networks and Learning Systems, 31(11), 4405–4423. https://doi.org/10.1109/TNNLS.2019.2957109
\bibitem{b20} Lu, D., \& Ricciuto, D. (2019). Efficient surrogate modeling methods for large-scale Earth system models based on machine-learning techniques. Geoscientific Model Development, 12(5), 1791–1807. https://doi.org/10.5194/gmd-12-1791-2019
\bibitem{b21} Lütjens, B., Crawford, C. H., Veillette, M., \& Newman, D. (2021). PCE-PINNs: Physics-Informed Neural Networks for Uncertainty Propagation in Ocean Modeling.
\bibitem{b22} Maslin, M. (n.d.) Climate : a very short introduction.
\bibitem{b23} Matthews, A. G. de G., van der Wilk, M., Nickson, T., Fujii, K., Boukouvalas, A., León-Villagrá, P., Ghahramani, Z., \& Hensman, J. (2016). GPflow: A Gaussian process library using TensorFlow. http://arxiv.org/abs/1610.08733
\bibitem{b24} Meinshausen, M., Raper, S. C. B., \& Wigley, T. M. L. (2008). MAGICC 6.0 Emulating IPCC AR4 atmosphere-ocean and carbon cycle models for projecting global-mean, hemispheric and land/ocean temperatures: MAGICC 6.0 MAGICC 6.0. In Chem. Phys. Discuss (Vol. 8). www.atmos-chem-phys-discuss.net/8/6153/2008/
\bibitem{b25} Morrison, P. (2004). The Discovery of Global Warming The Discovery of Global Warming Spencer R. Weart Harvard U. Press, Cambridge, MA, 2003. 24.95 (228 pp.). ISBN 0-674-01157-0. Physics Today, 57(6), 60–61. https://doi.org/10.1063/1.1784277
\bibitem{b26} Radhakrishnan Kristopher Rand Charles Stern Julius Busecke, A., Abernathey, R., Balaji, V., Kershaw, P., Privette, A., Stephens, A., Naik, N., Nikonov, S., Vahlenkamp, H., Blanusa, M., Banihirwe, A., Blanton, C., Perry Boh, N., Evans, B., Smith, R., Evans, R., Flamig, Z., Gergel, D., Jackson, T., … Sayibou, Z. (n.d.). CMIP6 Amazon-hosted Data Informational Session CMIP6 Data Informational session, Oct 13th, 2021 Community driven effort 4 Motivation: Nature. https://science.thewire.in/environment/what-the-ipcc-report-forecasts-for-india-development-future/
\bibitem{b27} Raissi, M., Perdikaris, P., \& Karniadakis, G. E. (2019). Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations. Journal of Computational Physics, 378, 686–707. https://doi.org/10.1016/j.jcp.2018.10.045
\bibitem{b28} Rajan, S. (2014). STATISTICAL DOWNSCALING OF GCM OUTPUT, HYDROLOGICAL SIMULATION AND GENERATION OF FUTURE SCENARIO USING VARIABLE INFILTRATION CAPACITY (VIC) MODEL FOR THE GANGA BASIN, INDIA.
\bibitem{b29} Reichstein, M., Camps-Valls, G., Stevens, B., Jung, M., Denzler, J., Carvalhais, N., \& Prabhat. (2019a). Deep learning and process understanding for data-driven Earth system science. Nature, 566(7743), 195–204. https://doi.org/10.1038/s41586-019-0912-1
\bibitem{b30} Reichstein, M., Camps-Valls, G., Stevens, B., Jung, M., Denzler, J., Carvalhais, N., \& Prabhat. (2019b). Deep learning and process understanding for data-driven Earth system science. Nature, 566(7743), 195–204. https://doi.org/10.1038/s41586-019-0912-1
\bibitem{b31} Satria Palar, P., Rizki Zuhal, L., \& Shimoyama, K. (2020a). Gaussian Process Surrogate Model with Composite Kernel Learning for Engineering Design. AIAA Journal, 58(4), 1864–1880. https://doi.org/10.2514/1.J058807
\bibitem{b32} Satria Palar, P., Rizki Zuhal, L., \& Shimoyama, K. (2020b). Gaussian Process Surrogate Model with Composite Kernel Learning for Engineering Design. AIAA Journal, 58(4), 1864–1880. https://doi.org/10.2514/1.J058807
\bibitem{b33} Wang, J. (2020). An Intuitive Tutorial to Gaussian Processes Regression. http://arxiv.org/abs/2009.10862
\bibitem{} Watson-Parris, D. (2020). Machine learning for weather and climate are worlds apart. https://doi.org/10.1098/rsta.2020.0098
\bibitem{} Watson-Parris, D., Williams, A., Deaconu, L., \& Stier, P. (n.d.). Model calibration using ESEm v1.0.0-an open, scalable Earth System Emulator.
\bibitem{} Watson-Parris, D., Rao, Y., Olivié, D., Seland, Ø., Nowack, P., Camps-Valls, G., Stier, P., Bouabid, S., Dewey, M., Fons, E., Gonzalez, J., Harder, P., Jeggle, K., Lenhardt, J., Manshausen, P., Novitasari, M., Ricard, L., \& Roesch, C. (2022). ETH Library ClimateBench v1.0: A Benchmark for Data-Driven Climate Projections Rights / license: Creative Commons Attribution 4.0 International Funding acknowledgement: 860100-innovative MachIne leaRning to constrain Aerosol-cloud CLimate Impacts (EC) ClimateBench v1.0: A Benchmark for Data-Driven Climate Projections Citation. Journal of Advances in Modeling Earth Systems, 14(10). https://doi.org/10.3929/ethz-b-000578488
\bibitem{} Weber, T., Corotan, A., Hutchinson, B., Kravitz, B., \& Link, R. (2020). Technical note: Deep learning for creating surrogate models of precipitation in Earth system models. Atmospheric Chemistry and Physics, 20(4), 2303–2317. https://doi.org/10.5194/acp-20-2303-2020
\bibitem{} Xu, W., Luo, X., Ren, Y., Park, J. H., Yoo, S., \& Nadiga, B. T. (2021). Feature Importance in a Deep Learning Climate Emulator.
\bibitem{}
\bibitem{}
\end{thebibliography}
\vspace{12pt}
\color{red}

\end{document}

